Space-Time Crop & Attend: Improving Cross-modal Video Representation Learning

The quality of the image representations obtained from self-supervised learning depends strongly on the type of data augmentations used in the learning formulation. Recent papers have ported these methods from still images to videos and found that leveraging both audio and video signals yields strong gains; however, they did not find that spatial augmentations such as cropping, which are very important for still images, work as well for videos. In this paper, we improve these formulations in two ways unique to the spatio-temporal aspect of videos. First, for space, we show that spatial augmentations such as cropping do work well for videos too, but that previous implementations, due to the high processing and memory cost, could not do this at a scale sufficient for it to work well. To address this issue, we first introduce Feature Crop, a method to simulate such augmentations much more efficiently directly in feature space. Second, we show that as opposed to naive average pooling, the use of transformer-based attention improves performance significantly, and is well suited for processing feature crops. Combining both of our discoveries into a new method, Space-Time Crop & Attend (STiCA) we achieve state-of-the-art performance across multiple video-representation learning benchmarks. In particular, we achieve new state-of-the-art accuracies of 67.0% on HMDB-51 and 93.1% on UCF-101 when pre-training on Kinetics-400.

==> STiCa (ICCV 2021)/1_introduction.tex <==
\section{Introduction}\label{s:intro}

\input{figs/fig-splash}

Visual representations have evolved significantly in the last two decades.
The first generation of representations comprises algorithms such as SIFT~\cite{lowe99object} and HOG~\cite{dalal05histogram} that were designed manually.
The second generation comprises representations learned from data by using deep neural networks and manual supervision~\citep{Krizhevsky12, deng2009imagenet,he16resnet}.
We are now transitioning to the third generation, where representations are learned from data without using any manual annotations by means of self-supervision.
Current self-supervised representations, obtained from methods such as MoCo~\cite{he2019momentum}, SimCLR~\cite{Chen2020ASF} or SwAV~\cite{caron2020swav}, convincingly outperform supervised ones on downstream tasks such as image classification, segmentation and object detection.
Furthermore, most of these methods are based on noise-contrastive instance discrimination, which was proposed in ExemplarCNNs~\cite{dosovitskiy2015discriminative} and put in its current form in~\cite{Wu_2018_CVPR} and~\cite{oord2018representation}.
The idea is to learn representations that are invariant to irrelevant factors of variations, modelled by strong augmentations such as image cropping, while remaining distinctive for the identity of the image.

Noise-contrastive learning is of course not limited to still images.
In particular, a number of recent approaches~\citep{miech2019endtoend, morgado2020avid, Patrick2020MultimodalSF, Han2020SelfsupervisedCF} have used noise-contrastive formulations to learn visual or audio-visual representations.
However, these methods are not as well developed as their counterparts for still images, with current state-of-the-art methods~\citep{Patrick2020MultimodalSF, Han2020SelfsupervisedCF} still lagging behind their supervised counterparts.

In this paper, we identify two areas in which current video representation learning formulations are lacking and improve on them, thus significantly improving upon the current state of the art in this area.

The first shortcoming is the lack of a sufficient encoding of \textbf{spatial invariances}.
For still images, learning spatial invariances has been shown to be one of the most important factors for performance~\citep{caron2020swav, Chen2020ASF}.
Almost all methods achieve some form of spatial invariance simply by applying different spatial augmentations to the images in different epochs of training.
However, learning spatial invariances in this manner requires a slow training process that lasts for many epochs ($\sim$800).
Authors have suggested that packing several augmentations of the same image in a single data batch is more effective as it provides a much stronger and more direct incentive for the network to learn invariances~\cite{caron2020swav}.

For videos, both strategies are less feasible.
Training a model for 200~epochs on Kinetics-400~\cite{kinetics} already requires around $1.5$K GPU hours on recent Nvidia V100 architectures, and with recent datasets such as IG65M~\cite{Ghadiyaram2019} and HowTo100M~\cite{miech19howto100m} only a handful of epochs can realistically be completed.
On the other hand, including multiple augmentations of the same video in a batch rapidly exhausts the memory of GPUs.
Since batch sizes per GPU are already in the single digits due to the size of video data, including several augmentations is unfeasible.
This is particular detrimental for recent contrastive learning approaches such as~\citep{he19momentum,Chen2020ASF}, where reducing the batch size means reducing the pool of negative contrastive samples.

% This is done primarily in two ways.
% The first approach is to induce spatial invariance by using different random spatial augmentations for each epoch of training.
% This allows the network to observe several transformed version of the same image; however, since an image is only observed once per epoch, the effect is small and the model need sto be trained fro a long time ($\sim$800~epochs)
% The second approach is to include multiple augmentations within each batch.
% In this way, the network can directly compare the representations obtained from several augmentations of the same data sample and learn to produce the same embedding for them~\cite{caron2020swav}.\footnote{In fact, methods such as SwAV leverage both approaches, training with multiple augmentations per batch, for 800~epochs.}

%
% that the network sees a large variety of transformed versions with the same target (e.g., a clustering pretext task), thus inducing invariance \textit{implicitly}.
% However, for videos, this is less feasible: training a model for 200~epochs on Kinetics-400~\cite{kinetics} already requires around $1.5$K GPU hours on recent Nvidia V100 architectures, and with recent datasets such as IG65M~\cite{Ghadiyaram2019} and HowTo100M~\cite{miech19howto100m} only a handful of epochs can realistically be completed.

% The second approach is to include multiple augmentations within each batch.
% In this way, the network can directly compare the representations obtained from several augmentations of the same data sample and learn to produce the same embedding for them~\cite{caron2020swav}.\footnote{In fact, methods such as SwAV leverage both approaches, training with multiple augmentations per batch, for 800~epochs.}
% Unfortunately, this quickly runs into the limits in terms of memory of GPUs: the cost of using multiple augmentations in a batch scales linearly with their number and quickly becomes infeasible for training video representations.
% Since batch sizes per GPU are already in the single digits due to the size of video data, including several augmentations in a batch is costly.
% Especially for recent contrastive learning approaches, reducing the batch size means reducing the pool of negative samples, which are crucial for performance~\cite{he19momentum,Chen2020ASF}.
% whereas contrastive formulation work much better when each batch also contains a large number of negatives to contrast against.
% to itraining models becomes even slower and with noise-contrastive learning even becomes infeasible as these require large number of negatives to contrast against.

In order to solve this problem, we propose to move spatial augmentations to the feature space, in a manner specifically tailored to contrastive learning.
Instead of extracting a large number $R$ of different augmentations in the input RGB space, we extract only two of them, apply the trunk of the neural network to extract corresponding features, and then extract $R/2$  more augmentations directly in feature space.
In this way, one needs to evaluate the slow and memory taxing feature extraction part of the network only twice, regardless of the number of augmentations that are produced.
We show that this \emph{feature-level augmentation} significantly improves  representation learning performance.
% the overall performance of the learned representation.

The second challenge that we tackle is how  to best encode \textbf{temporal information} in self-supervised video representation learning.
% While one may think that video representations should capture time well, most existing representations may fail do so.
Currently, most self-supervised video representation learning approaches use 3D-CNNs~\cite{Tran15, Tran18, I3D, xie2017rethinking} that compute convolutions across space and time, but the final representation is generated by na\"{\i}ve global average pooling over space and time, crucially discarding temporal ordering.

In order to address this shortcoming, in this work we propose to use a contextualized pooling function based on the transformer architecture~\cite{vaswani2017attention} for both self-supervised pretraining and supervised finetuning.
The intuition is that, via multi-head self-attention, the transformer can capture temporal dependencies much better than average pooling, especially for longer inputs.
Transformers can also benefit from our feature-level crops, as the latter resemble the common approach of randomly masking the inputs to the transformer~\cite{bert18}.
Experimental results show that this modification improves the performance of the learned video representations substantially, and is cumulative with the benefit of feature crops, at about the same cost of average pooling.

We combine both of our proposed improvements into a new self-supervised learning approach: Space-Time Attention and Cropping (\textbf{\methodname}).
To summarize, with \methodname{} we make the following three main contributions:
\begin{itemize}
\item We demonstrate the benefits of stronger spatial invariances in self-supervised video representation learning for the first time  and we propose feature-level augmentation to implement the latter efficiently.
\item We propose to use transformers to model time more effectively in self-supervised video representations, replacing average as the pooling function.
\item We demonstrate strong performance gains by using the two techniques and obtain state-of-the-art performance on two standard benchmarks ($67.0\%$ on HMDB-51 and $93.1\%$ on UCF-101).
\end{itemize}



==> STiCa (ICCV 2021)/2_related_work.tex <==
\section{Related Works}
\paragraph{Self-supervised Image Representation Learning.}
Self-supervised learning uses pretext tasks to automatically and easily generate differentiable learning signals from the data itself in order to train convolutional neural networks.
A variety of pretext tasks have been proposed such as colorization~\citep{zhang2016colorful, zhang2017split}, predicting artificial rotations~\citep{gidaris2018unsupervised}, in-painting~\citep{pathak2016context}, spatial context~\citep{doersch2015unsupervised, noroozi2016unsupervised}, and clustering features~\citep{caron2018deep, caron2019unsupervised, ji2018invariant, asano2020self, li2020prototypical, caron2020swav}.
Recently, contrastive methods~\citep{Hadsell2006DimensionalityRB, gutmann2010noise} have proven to be particularly effective at learning transferable image representations~\citep{he2019momentum, bachman2019learning, misra2019selfsupervised, Chen2020ASF, grill2020bootstrap, tian2019contrastive, oord2018representation}.

\paragraph{Self-supervised Video Representation Learning.}
For videos, pretext tasks often seek to leverage the temporal dimension to learn representations. 
Such tasks include predicting clip and sequence order~\citep{clip_order, lee2017unsupervised, misra2016shuffle}, future events~\citep{han2019video, Han2020MemoryaugmentedDP}, the arrow of time~\citep{wei2018learning}, 3D geometric transformations~\citep{jing2018self, kim2019self}, playback speed~\citep{benaim2020speednet, Wang2020SelfsupervisedVR, Jenni2020VideoRL, Epstein2020OopsPU}, or motion
statistics~\citep{motion_statistics}. 

\paragraph{Multi-Modal Learning.}
The co-occurrence and synchronicity of multiple modalities from videos have been used to learn visual representations from both audio-video~\citep{Arandjelovic17, owens2018audio, avts, alwassel2019self, morgado2020avid, Patrick2020MultimodalSF, asano2020labelling, ma2020learning}, and speech-video~\citep{miech17learning, sun2019videobert, sun2019contrastive, miech2019endtoend, nagrani2020, li2020learning, korbar2020video, alayrac2020selfsupervised, patrick2020supportset, Stroud2020LearningVR} data. 
Multi-modal representation learning has several practical applications: lip reading~\citep{Chung16a, Chung_2017_lip_reading, afouras2018deep_lip_reading}, audio-visual source separation and localization~\citep{arandjelovic2018objects, zhao2018sound, afouras2018conversation, zhao2019sound, harwath2018jointly, Afouras2020SelfSupervisedLO}, speech recognition~\citep{potamianos2003recent, afouras2018deep}, efficient inference~\citep{gao2019listen, korbar2019scsampler}, egocentric action recognition~\citep{kazakos2019epicfusion} and audio-visual navigation~\citep{chen2019audiovisual}.

\paragraph{Data Augmentations.}
Data augmentation has proven to be useful in training deep learning models in many domains, from vision~\citep{autoaugment, Cubuk2019RandAugmentPD, yun2019cutmix} to speech~\citep{Park2019SpecAugmentAS}.
Data transformations are the foundation of most self-supervised works, and there has been early attempts to even learn the optimal distribution of transformations~\citep{buchler2018improving,autoaugment}. 
Particularly for contrastive learning, the choice of data transformations has been shown to be particularly important to learn desirable invariances and equivariances~\citep{misra2019selfsupervised, Patrick2020MultimodalSF, tian2019contrastive, tian2020makes}.
% It is also possible to generate new harder negatives used for constrastive learning in the feature-space directly~\citep{kalantidis2020hard}.
%Transformations can also be done in the feature space~\citep{kalantidis2020hard} to make harder negatives in contrastive learning. 

\paragraph{Transformations in Feature-Space.}
Some works have proposed forms of augmentation in feature-space, by adding noise and linear transformations~\citep{terrance2017dataset}, and by associating samples to prototypes in feature-space~\citep{kuo2020featmatch}. These augmentations do not correspond to interpretable geometric operations, however.
Crops in feature-space are commonly used in supervised detection pipelines, such as Faster R-CNN and region-based architectures~\citep{ren2015faster}, and in earlier detectors based on manually-engineered features~\citep{dalal05histogram}. However, the objective of these transformations is to enumerate a space of outputs (e.g. bounding box predictions) for supervised prediction. 
In self-supervised learning, while~\citep{kalantidis2020hard} uses feature mixing to create harder negatives for contrastive learning, we are instead interested in using feature crop augmentation to achieve spatial invariance.

\paragraph{Temporal Modeling.}
Videos extend images by adding a temporal dimension.
Therefore, there has been a large family of research that has looked into how to model temporal information in videos. 
Early works incorporated temporal information via average pooling of frame/clip-level features~\citep{Sports1M, wang16temporal, Girdhar17}, while later work used 3D convolution neural networks~\citep{Tran15, Tran18, xie2017rethinking} and recurrent-neural networks~\citep{donahue2016longterm}. 
Other approaches leverage long-term temporal convolutions~\citep{varol17}, self-attention~\citep{XiaolongWang18}, relation networks~\citep{abs08496}, multi-scale temporal convolutions~\citep{hussein2019timeception}, or optical flow in a two stream network~\citep{simonyan2014twostream}. 

\paragraph{Transformers in Vision.} 
With the success of the transformer architecture~\citep{vaswani2017attention} in natural language processing~\citep{bert18}, transformers are being used in various vision domains such as image representation learning~\citep{dosovitskiy2020image, chen2020generative, wu2020visual, desai2020virtex, sariyildiz2020learning}, image generation~\citep{parmar2018image}, object detection~\citep{locatello2020objectcentric, carion2020endtoend}, few-shot learning~\citep{doersch2020crosstransformers}, video action recognition~\citep{XiaolongWang18, girdhar2019video,timesformer,neimark2021VTN}, video question-answering~\citep{kant2020spatially}, image-text~\citep{lu2019vilbert, su2019vlbert, Tan_2019, li2019visualbert, tan2020vokenization} and video-text~\citep{sun2019videobert, sun2019contrastive, zhu2020actbert, gabeur2020multimodal, patrick2020supportset, korbar2020video} representation learning. 

==> STiCa (ICCV 2021)/3_methods.tex <==
\section{Method}\label{s:method}

\input{figs/fig-method}

\newcommand{\bx}{{\bm x}}
\newcommand{\by}{{\bm y}}
\newcommand{\bz}{{\bm z}}
\newcommand{\bw}{{\bm w}}
\newcommand{\bv}{{\bm v}}
\newcommand{\ba}{{\bm a}}
\newcommand{\bh}{{\bm h}}

Our goal is to learn a general-purpose \emph{data representation} $\Phi : \mathcal{X} \rightarrow \mathcal{Z} = \mathbb{R}^D$ that maps data $\bx\in\mathcal{X}$ to feature vectors $\bz=\Phi(\bx)$.
In the supervised setting, representations are learned end-to-end as components of larger systems that solve certain tasks of interest, such as image or video classification, under the assumption that supervision is available to drive the learning process.
When supervision is not available, representations can still be learned via self-supervision by means of suitable pretext tasks.
Among the latter, \emph{noise contrastive learning} is one of the most popular and successful ones~\citep{oord2018representation,Chen2020ASF}.
We summarize this background next and discuss our extensions in the following sections.

\subsection{Background: Multi-modal contrastive learning}

The idea is to train the representation $\Phi$ to identify data points up to the addition of noise or, more generally, the application of certain nuisance transformations.
To this end, let $g : \mathcal{X} \rightarrow \mathcal{X}$ be transformations sampled in a set $\mathcal{G}$ of possible nuisances (for example random image crops).
Let $\operatorname{sim}(\bz',\bz'')$ be a similarity function comparing representations $\bz'$ and $\bz''$, such as the cosine similarity:
$$
\operatorname{sim}(\bz',\bz'')
=
\frac
{\langle\bz', \bz''\rangle}
{\|\bz'\| \, \|\bz''\|}.
$$
Consider a dataset or batch $\mathcal{B} = \{\bx_1,\dots,\bx_N\}$ of data samples.
Slightly modifying~\citep{Chen2020ASF}, for each sample $\bx_i$, draw a set of random nuisance transformations 
$
\{ g_{\alpha i}\}_{1\leq i \leq N}
$
and let
$
\bz_{\alpha i}= \Phi(g_{\alpha i}(\bx_{i}))
$
be the representations of the transformed samples.
Likewise, consider a second set $\beta$ of transformations
$
\{ g_{\beta i}\}_{1\leq i \leq N}.
$
% Define
% $
% \bz_{\kappa i}= \Phi(g_{\kappa i}(\bx_{i}))
% $
% to be the representations of the transformed samples.
The noise contrastive loss (NCE) is given by:
\begin{equation}\label{eq:contrastive}
\mathcal{L}(\alpha,\beta)
=
-\frac{1}{N}
\sum_{i=1}^N
\log \frac
{e^{\frac{1}{\tau}\operatorname{sim}(\bm z_{\alpha i}, \bm z_{\beta i})}}
{
\sum_{j=1}^N
e^{\frac{1}{\tau}\operatorname{sim}(\bm z_{\alpha i}, \bm z_{\beta j})}
}
\end{equation}
where $\tau > 0$ is a temperature parameter.
This loss pulls together the representations of samples that only differ by the transformation while pushing apart the others.
Note that this definition is not symmetric in the two arguments $\alpha$ and $\beta$ (i.e., $\mathcal{L}(\alpha,\beta)\not=\mathcal{L}(\beta,\alpha)$.
Note also that we can introduce any number of transformation sets $\alpha,\beta,\gamma,\dots$ and, for each pair, we can obtain a different variant of~\cref{eq:contrastive}.

% Note that, differently from other works~\citep{Chen2020ASF}, our definition is \emph{not} symmetric, in the sense that
% $
% \mathcal{L}(\kappa_1,\kappa_2)
% \not=
% \mathcal{L}(\kappa_2,\kappa_1).
% $
% We can interpret this as follows:
% the first transformation set $\alpha$ is used to generate a `query' and the second transformation set $\beta$ is used to generate `keys';
% \cref{eq:contrastive} rewards finding each query in the keys despite the fact that the applied transformation is different.
% The advantage of this asymmetric variant or the NCE loss is that it supports certain efficient formulations introduced later.

% When the data $\bx$ consists of images, typical nuisance transformations include random cropping and color jittering.
Recently, works such as~\citep{Patrick2020MultimodalSF} have ported this technique to the video domain
% , thus operating with multi-modal signals.
% The key ingredient is to decompose 
by contrasting modalities.
Each video $\bx=(\bv,\ba)$ consists of a visual component $\bv$ and an audio component $\ba$.
One consider two sets of transformations $g_v$, extracting and augmenting the visual component, and $g_a$, extracting and augmenting the audio component.
We still write $\Phi(g_\alpha(\bx))$ for the feature computed for either visual and audio components, but the symbol means that a modality-specific neural network is applied as needed.\footnote{
In other words, $\Phi = (\Phi_v,\Phi_a)$ is really a pair of networks, producing embedding vectors $\bz_\alpha$ that are compatible regardless of the modality $\alpha \in \{v,a\}$.}


With this, we can derive three variants of~\cref{eq:contrastive}, involving mixed visual-audio and homogeneous visual-visual and audio-audio comparisons.
Their combinations are:
\begin{equation}\label{eq:multi-loss}
\lambda_{va} \mathcal{L}(v, a) +
\lambda_{av} \mathcal{L}(a, v)
+ \lambda_{vv} \mathcal{L}(v_1, v_2) +
\lambda_{aa} \mathcal{L}(a_1, a_2).
\end{equation}
% Unpacking this notation, the first term amounts to considering representations $\bz_{vi}=\Phi(g_{vi}(\bx_i))$ and $\bz_{ai}=\Phi(g_{ai}(\bx_i))$ where $g_{v1},\dots,g_{vN}$ are $N$ visual transformations and $g_{a1},\dots,g_{aN}$ are $N$ audio transformations.
% These expressions can be plugged in~\cref{eq:contrastive} directly.
% The second term in~\cref{eq:multi-loss} is similar, but considers pairs of video transformations $g_{v_1i}$ and $g_{v_2i}$ for each data sample $\bx_i$.
% The third term is like the second, but for audio.
where
$\lambda_{va}$,
$\lambda_{av}$,
$\lambda_{vv}$ and
$\lambda_{aa}$ are non-negative mixing weights.

% The loss is

% \subsection{Preliminaries: Noise-Contrastive Learning}
% An approach that has gained popularity for its simplicity and performance is noise-constrastive learning~\citep{oord2018representation, Chen2020ASF}.
% Here, feature representations are trained such that an a modified input $x_i'$ can be re-identified against other "noise" samples $x_j, j\neq i$.
% In practice, these modifications to the input are common augmentation methods such as random cropping, or color jittering and provide the network with enough signal to learn invariance against these nuisance factors, as well as learn variance against stable features of inputs.
% The loss is

\paragraph{Challenge 1: Encoding within-modality invariance.}

While all terms in \ref{eq:multi-loss} code for desirable invariances of the representation, several recent papers~\citep{Patrick2020MultimodalSF, morgado2020avid, ma2020learning} have found that the mixed term $\lambda_{va}$ is far more important than the other two; in fact, performance \emph{degrades} if one sets $\lambda_{aa},\lambda_{vv} \neq 0$, meaning that within-modal invariances are not successfully leveraged.
%it is preferable to only retain the cross-modal training signals.
%
% We can explain the importance of 
% Contrasting different modalities is a good proxy for abstraction, but
% (as an any factor that correlates images and sounds, such as an object category, is likely to be an abstract one).
% However,
% this does not explain why coding also for within-modality invariances should not help.
Our hypothesis is that within-modality invariance can be beneficial, and that these early negative results are due to the fact that current learning formulations are ineffective at capitalizing on this signal.

As suggested in~\cref{s:intro}, the fact that video data is large means that the batch size used in learning must be small.
As a consequence, a batch can contain only a very small number of different augmentations of the same video sample.
%  which is however very beneficial to learn a specific invariance.
In current multi-modal learning formulations, each video is already transformed twice in order to extract video and audio components, so cross-modal invariance is learned well.
However, the downside is that there is no space left in the batch for multiple visual or audio augmentations.
Thus, within-modality invariance is learned only indirectly --- in particular, as noted in~\cref{s:intro}, two different visual or audio augmentations of the same video are visited by the model only after an entire training epoch.
% For very large datasets such as IG65M, this happens at most a few times during the whole training process.
% The main issue is that, by focusing exclusively on this signal comes at the expense of explicitly learning invariance in each single modality.
% This is because, in order to observe two different visual/audio augmentations of a given data sample, one needs to wait for en entire epoch for that data point to be sampled again.
% By comparison, sampling and contrasting two different visual/audio augmentations of the same video in the same batch should encourage the model to learn corresponding invariances much faster.
Next, we address this issue by making it feasible to extract several within-modality transformations in the same batch even for video data.

% can only be implicitly learned by sampling a difference transformation at every training epoch.
% However, ever larger datasets (such as IG65M) mean that one training run might see each example only a handful of times.
% Thus, current NCE-based methods cannot fully leverage single-modal training signals.

% In this work, we tackle this issue from two sides.
% First, we develop a novel spatial invariance enforcing scheme that improves performance while being highly efficient.
% Second, we improve the modelling of time in our network, thus allowing it to learn stronger representations that can leverage time as a variant signal.

\subsection{Efficient spatial cropping for augmentation}\label{s:featurecrop}

% We conjecture that the reason why within-modality augmentation has so far been ineffective in multi-modal self-supervision is not an intrinsic limitation of the approach, but rather the result of practical limitation arising from the computational cost of doing so at the required scale when videos are considered.
It has been found that self-supervised learning benefits from, and requires more and stronger augmentations compared to the supervised counterpart for optimal performance~\citep{Chen2020ASF}.
In particular, several papers~\citep{Chen2020ASF,asano2020a,caron2020swav} have suggested that, in the case of still images, the most important type of augmentation is \emph{cropping}. 
% Starting from still images, while several algorithms have been proposed for self-supervised learning on such data, much of the final performance does not depend so much on the specific algorithm but on the choice of image transformations $t$ used for augmentation~\citep{Chen2020ASF,asano2020a}.
% Among those, the most important is likely \emph{cropping}.
Namely, given an RGB image $\bx \in \mathbb{R}^{3  \times H \times W}$ with three channels and height and width $H$ and $W$ respectively, a crop is given by a box $B=(x_\textrm{min},x_\textrm{max},y_\textrm{min},y_\textrm{max})$.
The image tensor is first cropped as:
\begin{equation}\label{e:imcrop}
    C_B(\bx) =
    \bx_{[:,~
    y_\textrm{min}:y_\textrm{max},~
    x_\textrm{min}:x_\textrm{max}]}
\end{equation}
where the $:$ symbol is used to denote an index range.
The cropped tensor is then resized to a tensor
$
\tilde\bx = g(\bx) = R_{H_0W_0}(C_B(\bx)) \in \mathbb{R}^{3\times H_0\times W_0}
$
with a given height and width $H_0\times W_0$.
In practice, $R_{H_0W_0}$ may also apply additional augmentations such as color jittering, as detailed in the experiments.

As for the visual part $\bv \in \mathbb{R}^{3\times T\times H\times W}$ of a video, the situation is similar, except that the video also contains an additional temporal dimension $T$.
To avoid extreme spatial jittering and keep objects aligned, a spatial crop is usually taken at the same location in the input space throughout the whole temporal dimension, so we consider the tube
$
B =
(
    x_\textrm{min},x_\textrm{max},
    y_\textrm{min},y_\textrm{max},
    t_\textrm{min},t_\textrm{max}
)
$
and define
$
\tilde \bv = g_v(\bv) = R_{H_0W_0}(C_B(\bv)) \in \mathbb{R}^{3 \times T_0 \times H_0 \times W_0}
$
by extending~\eqref{e:imcrop} in the obvious way.
% TODO: presumably the frame rate never changes so there is no time-resize?

% First, the a crop $C(I)$ is taken such that $C(I) = I^{[x_\textrm{min}:x_\textrm{max},y_\textrm{min}:y_\textrm{max}]}$, with crop-box coordinates $x_i,y_i$ chosen to satisfy aspect-ratio and scale constraints.
% Here, the height and width of the crop are different from the original: \mbox{$H(C(I)){=}y_\mathrm{max}-y_\mathrm{min}{\neq} H(I)$} and $W(C(I)){\neq} W(I)$.
% For simplicity, we now drop the usage of width $W$ as it always follows that of the height $H$.
% Following this, the inputs are resized to form a fixed input size to allow for efficient batching and computation, such that the size of the resulting transformed images $I'$ are constant: $H(I) = H(I') = H(R(C(I)))$.

% \subsection{Feature Box Cropping \label{s:meth:crops}}
% Cropping has been shown to be the key augmentation for self-supervised learning~\citep{Chen2020ASF,asano2020a}.
% As such, it can provide the model the learning signal of spatial invariance, as well as regularising the training by strongly increasing the input data diversity.
% Typical cropping methods act in the input domain such as RGB image $I \in \mathbb{R}^{3  \times H \times W }$ and contain two parts: a crop-selection $C$ and a resize operation $R$.
% First, the a crop $C(I)$ is taken such that $C(I) = I^{[x_\textrm{min}:x_\textrm{max},y_\textrm{min}:y_\textrm{max}]}$, with crop-box coordinates $x_i,y_i$ chosen to satisfy aspect-ratio and scale constraints.
% Here, the height and width of the crop are different from the original: \mbox{$H(C(I)){=}y_\mathrm{max}-y_\mathrm{min}{\neq} H(I)$} and $W(C(I)){\neq} W(I)$.
% For simplicity, we now drop the usage of width $W$ as it always follows that of the height $H$.
% Following this, the inputs are resized to form a fixed input size to allow for efficient batching and computation, such that the size of the resulting transformed images $I'$ are constant: $H(I) = H(I') = H(R(C(I)))$.

% \subsubsection{Videos}
% Compared to images, a  video $V$ contains an additional temporal dimension $T$.
% Thus, for the visual modalities our inputs are of size $V \in \mathbb{R}^{3  \times T \times H \times W }$, with input frames $T$ that typically cover 1 or 2 seconds.
% To allow avoid extreme spatial jittering and keep objects aligned, a spatial crop is usually taken at the same location in the input space throughout the whole temporal dimension.

The deep neural network $\bz = \Phi(\tilde\bv)$ mapping $\bv$ to its corresponding code $\bz$ is fed with tensors with two spatial dimensions and a temporal one.
Such networks, often called 3D for this reason, include R3D~\citep{hara2017learning}, S3D~\citep{xie2017rethinking} and R(2+1)D~\citep{Tran18}.
As customary in deep convolutional neural networks, they first produce an intermediate tensor with lower space-time resolution and then pool the latter to obtain a single code vector for the entire video.
We explicitly break this down into three functions
\begin{equation}\label{e:decomp}
    \Phi(\tilde\bv) = (\mathcal{P}_t \circ \mathcal{P}_{s} \circ \Psi)(\tilde\bv)
\end{equation}
Here, the first function is a 3D convolutional neural network
$
\Psi(\tilde\bv) \in \mathbb{R}^{D \times T_1 \times H_1 \times W_1}
$
producing a tensor with reduced resolution $T_1<T_0$, $H_1<H_0$, $W_1<W_0$.
The operators $\mathcal{P}_{s}$ and $\mathcal{P}_t$ collapse, respectively, \underline{s}patial and \underline{t}ime dimensions via average pooling.

Now consider implementing term $\mathcal{L}(v_1,v_2)$ in~\ref{eq:multi-loss}.
In this case, one samples from each video $\bx_i$ two different space-time crops $g_{v_1i}(\bx_i)$ and $g_{v_2i}(\bx_i)$, each corresponding to random tubes $B_1$ and $B_2$ respectively.
The tubes are not sampled entirely independently, however, as they have the same temporal extent $(t_\textrm{min},t_\textrm{max})$.

\paragraph{Na\"{\i}ve multiple spatial cropping} % are too expensive.}

In practice, \citep{caron2020swav, Chen2020ASF, li2020centerwise, misra2019selfsupervised} show that taking multiple image crops improves self-supervised image representations.
We can achieve a similar effect for videos by summing losses 
$
\mathcal{L}(v_\alpha,v_\beta)
$
for sets of visual transformations $v_\alpha \not= v_\beta$, obtained by sampling multiple space-time tubes for each video, but this is practically difficult, both due to the large memory footprint and the compute overhead of the slow 3D CNN for each crop.
% First, since the input data are already much larger than for images (due to the temporal dimension), taking multiple crops can only be done if the batch size $N$ is also reduced, which hinder contrastive learning considerably by reducing the number of negatives.
% Second, computing features $\Phi(g_{v_\alpha i}(\bv_i))$ for a large number of different crop sets $\alpha$ is very time consuming as a complex 3D CNN must be applied form scratch on top of each crop computed.

The Multi-Crop approach introduced by SwAV~\citep{caron2020swav} in the image domain combined with our asymmetric contrastive formulation~\eqref{eq:contrastive} can partially reduce the complexity.
For Multi-Crop, we consider three crop sizes $\alpha \in \{L_1,L_2,S\}$ where $L_1$ and $L_2$ stands for large and $S$ for small.
The use of a small crop allows to reduce the memory consumption when the representation $\Phi$ is computed.
We then have losses:
$$
\mathcal{L}(v_{L_1},v_{L_2})
+\mathcal{L}(v_{L_2},v_{L_1})
+\mathcal{L}(v_{L_1},v_{S})
+\mathcal{L}(v_{L_2},v_{S}).
$$
While operating on small videos saves some computation, in practice this approach is insufficient to allow using more than a handful of crops in total.

\paragraph{Efficient cropping in feature space.}

As illustrated in~\cref{fig:short}, a much more efficient alternative to cropping the input video is to crop intermediate features. 

To do so, we first apply the trunk $\Psi$ of the representation to an input-space crop of the visual component of the video $\tilde \bv = R_{H_0W_0}(C_B(\bv))\in\mathbb{R}^{D\times T_1\times H_1\times W_1}$.
Then we can efficiently construct a new view of this data by applying the \textit{Feature Crop} $C_{\bar B}$ directly on each intermediate representation, yielding
\begin{equation}\label{e:featurecrop}
    \bar \bv =
    C_{\bar B}(\Psi(\tilde \bv))  =   \Psi(\tilde \bv)_{[
    t_\textrm{min}:t_\textrm{max},~
    y_\textrm{min}:y_\textrm{max},~
    x_\textrm{min}:x_\textrm{max}]}
\end{equation}
Since the operator $C_{\bar B}$ is lightweight, it can be used to compute several such random views efficiently;
by comparison, cropping the input RGB images requires recomputing the trunk $\Psi$  multiple times.
% We can, in this manner, produce a large number $J$ of cheaply computed spatial \textit{and} temporal crops $\bar \bv$ out of a single RGB tube $\tilde \bv$, saving on recomputing the trunk $\Psi$ multiple times.

In practice, given an input video $\bv$, we generate the following views.
First, we apply two crops in RGB space, producing two large crops $L_1$ and $L_2$.
Then, for each of those, we use the operator~\eqref{e:featurecrop} to generate $m$ medium-sized and $n$ small-sized crops
$
\mathcal{T}_i =
\{M_1 L_i, \dots, M_m L_i, S_1 L_i, \dots, S_n L_i\}
$.
We define an overall within-modality loss by summing losses for each pairs of views in $\mathcal{T}$ with exception of pairs where both crops are small:
% $
% \mathcal{S}_i
% =
% \{S_1 L_i, \dots, S_n L_i\}
% $,
\begin{multline}\label{e:lossvisual}
L_{vv}
=
\sum_{\alpha,\beta}
\mathcal{L}(v_\alpha, v_\beta)
+
\mathcal{L}(v_\beta, v_\alpha),
 ~~~ \text{where}
\\
(\alpha,\beta) \in 
(\mathcal{T}_1\times \mathcal{T}_2) - (\mathcal{S}_1\times \mathcal{S}_2)
% \end{cases}
\end{multline}
Note that there are $2((m+n)^2-n^2)$ terms in this loss.
This is a far greater number of comparison than afforded by the two initial input-space RGB crops.

% \paragraph{Receptive Field of Feature Crops and Preventing Shortcut Learning.} Noise contrastive learning works better when you can reduce the mutual information between the input pairs~\citep{tian2020makes} as its harder for the network to cheat. 
% This can be achieved by taking multiple spatial crops of images in the input space and independently applying different augmentations, such as color jittering and Gaussian blurring, to the cropped inputs.
% However, as mentioned above, taking more than 2 crops in input space is both memory and computationally infeasible for multi-modal video data.
% Crops in feature space, on the other hand, allows us to take multiple crops for noise contrastive learning. 
% However, since CNNs have large receptive fields that easily cover the full frame, there may be shortcut learning with feature crops as information may leak between the crops from same feature map.
% To alleviate this, we take feature crops from two originally augmented video clips, allowing us to make NCE comparisons \emph{across} modalities and individual augmentations (such as color jitter), leading to a beneficial reduction in mutual information.
% Furthermore, while the theoretical receptive fields of units in later layers are indeed very large, units tend to be sensitive to an effective area which is significantly smaller than the theoretical receptive field~\citep{luo2017understanding, ZhouKLOT14}, further reducing the mutual information between inputs for noise contrastive learning.

% In practice, we consider two sets of feature crop sizes, small 
%$(\bar{S}_1,\bar{S}_2)$
% \\
% d large %$(\bar{L}_1,\bar{L}_2)$ 
% for both intermediate features $\Psi(\bar{\bv}_1),\Psi(\bar{\bv}_2)$. 
% Thus, for each original RGB-space crop $i{=}1,2$ we have have set of different spatial features $T_i = \{( \bar S_1,\dots  \bar S_N),( \bar L_1,\dots,  \bar L_M)\} := \{\underline{S}_i, \underline{L}_i \}$. 
% % Note the difference to the previous section, where now each $\bar{C}$ is a set of crops of size $C$ instead of being a single crop.
% Next, when computing the losses, we only allow noise-contrastive comparisons between features of the different initial views. 
% This is to account for the fact that the receptive fields of the backbones are large and even taking non-overlapping crops in feature space, results in highly similar features.
% This is solved by sampling two initial views and comparing only across these.
% Thus, since noise-contrastive learning only requires pair-wise comparisons, we only need a constant number of 2 initial crops to generate any number of intermediate crops, highlighting the efficiency and scalability in using feature box crops for learning invariances.
% Finally, we also follow~\citep{caron2020swav} in not computing small to small comparisons for comparability. 
% Thus, the within-modality loss can be computed as:
% \begin{equation}\label{e:lossvisual}
% L_v
% =
% \sum_{\alpha,\beta}
% \mathcal{L}(v_\alpha, v_\beta), 
% \quad 
% % ~~\text{with}~~
% % \begin{cases}
% % \alpha \in \{\bar{L}_1,\bar{L}_2\},\\
% % \beta \in \{\bar{L}_1,\bar{L}_2,\bar{S}_1,\bar{S}_2\},\\
% (\alpha,\beta) \in \{ T_1 \! \times \! T_2 \} \setminus  \{ \underline{S}_1 \! \times \! \underline{S}_2 \}
% % \end{cases}
% \end{equation}

% In particular, we take crops in the feature space $C^\mathrm{f}=  C^\mathrm{s} \times C^\mathrm{t}$ that consist of cropping in the spatial
% \begin{align}
%    C^\mathrm{s}(\Phi(V)) &= \Phi(V)^{[:,  x_\textrm{min}:x_\textrm{max},y_\textrm{min}:y_\textrm{max}, :]}
% \end{align}
% and temporal domain
% \begin{align}
% C^\mathrm{t}(\Phi(V)) &= \Phi(V)^{[t_\textrm{min}:t_\textrm{max}, :, :, :]}.
% \end{align}
% Here, `$:$' stands for not computing a crop in that dimension.

% Thus, using our feature space cropping method, can yield a set of augmented features $\mathcal{S}_f(V)$ as:
% \begin{align}
%     \mathcal{S}_f(V) = \{ \mathcal{P}(C^\mathrm{f}_1(\Phi_V), C^\mathrm{f}_2\Phi_V, \dots)\},
% \end{align}
% where $\Phi_V=\Phi(V)$ is the penultimate representation that is recycled for computing crops, which allows us to only use a single forward pass.


% Inspired by works in the image domain such as SwAV~\citep{caron2020swav}, we take two distinct sets of sizes for the feature-box crops for both the spatial and the temporal dimension, one small $C^{\mathrm{f,S}}$ and one large $C^{\mathrm{f,L}}$.
% In particular, in addition to the cross-modal loss used in~\eqref{eq:loss}, we compute noise-contrastive losses within the visual modality, we thus have $\lambda_2 = \lambda_3 = \lambda_4 = 1$.
% To compute the visual modality loss $L(v_i,v_j)$, we form pairs of dot products of the form $ \langle f(C^{\mathrm{f,S}}), f(C^{\mathrm{f,L})} \rangle$ and $ \langle f(C^{\mathrm{f,L}}), f(C^{\mathrm{f,L}}) \rangle$, where $f(C)$ denotes the application of feature-box crop $C$ on a video's representation and the subsequent computation of the embedding.
% In addition, in practice we always apply the crops on which losses are computed on two different original augmented versions of the video, ie. $ \langle f(C_2(v)), f(C_1(v')) \rangle$.
% While this does increase the compute time, it crucially does not scale with the amount of crops taken in the feature space.
% This is in stark contrast to cropping in the input domain where taking $N$ crops results in a slowdown proportional to $N$.


% \subsubsection{Cropping in feature space}
% With increasing depth, video architectures such as R3D~\citep{Tran18}, S3D~\citep{xie2017rethinking} and R(2+1)D~\citep{Tran18} all gradually reduce spatial and temporal dimensions.
% This is done until the final layer, which is preceeded by a global pooling operation $\mathcal{P}$ that reduces both spatial and temporal dimensions to 1, leaving a single feature vector.
% More formally, let $\Phi(V) \in \mathbb{R}^{3 \times t \times h \times h}$ be the penultimate representation for a video $V$, with embedding dimensions $t<T$, $h<H$, $w<W$.
% The final representations is then given by $\mathcal{P}(\Phi(V)) \in \mathbb{R}^{d \times 1 \times 1 \times 1}$.
% Therefore, a naive application of cropping for videos can be achieved by first producing cropped variants $\{C_1(V),C_2(V), \dots \}$ of an input and subsequently computing multiple forward passes through the network, yielding the set of features $\mathcal{S}(V)$ for video V:
% \begin{equation}
% \mathcal{S}(V) =  \{ \mathcal{P}(\Phi(C_1(V)),\mathcal{P}(\Phi(C_2(V)), \dots)\})
% \end{equation}

% While taking multiple crops for augmenting an image yields consistent benefits and has been used in recent self-supervised image representations works~\citep{caron2020swav, Chen2020ASF, li2020centerwise}, for videos, this quickly becomes infeasible due to two reasons.
% First, since the input data are already much larger than for images (due to the temporal dimension), taking multiple crops leads to quickly decreasing batch sizes, which hinder learning methods such as contrastive learning considerably by reducing the number of negatives.
% Second, the doubling of training time is exacerbated for video representation learning where each run can take up to ($64\! \cdot \! 3 \!=\!192$ GPU days).


% In order to still encode invariances induced by cropping, we propose to make use of the spatial and temporal extent left in the  pen-ultimate representations $\Phi(V)$.
% In particular, we take crops in the feature space $C^\mathrm{f}=  C^\mathrm{s} \times C^\mathrm{t}$ that consist of cropping in the spatial
% \begin{align}
%    C^\mathrm{s}(\Phi(V)) &= \Phi(V)^{[:,  x_\textrm{min}:x_\textrm{max},y_\textrm{min}:y_\textrm{max}, :]}
% \end{align}
% and temporal domain
% \begin{align}
% C^\mathrm{t}(\Phi(V)) &= \Phi(V)^{[t_\textrm{min}:t_\textrm{max}, :, :, :]}.
% \end{align}
% Here, `$:$' stands for not computing a crop in that dimension.

% Thus, using our feature space cropping method, can yield a set of augmented features $\mathcal{S}_f(V)$ as:
% \begin{align}
%     \mathcal{S}_f(V) = \{ \mathcal{P}(C^\mathrm{f}_1(\Phi_V), C^\mathrm{f}_2\Phi_V, \dots)\},
% \end{align}
% where $\Phi_V=\Phi(V)$ is the penultimate representation that is recycled for computing crops, which allows us to only use a single forward pass.

\subsection{Temporal modelling with transformers}\label{s:meth:transformer}

% In the previous section, we have discussed how to obtain better spatial/crop invariance when modelling videos.
% Here, we note that improvements are also possible on how time is captured by the model.
% In particular, most current video architectures do not fully exploit the temporality of the encoded features.

We now discuss our second improvement: better modelling of time.

\paragraph{Challenge 2: Modelling time better.} 

Contrary to spatial invariance, models should not be fully invariant to time as the latter can encode causality and with it semantics: a video of someone starting a fire is very different from its reversed version, in which someone extinguishes it.
%
In standard 3D networks, features in the trunk are sensitive to the temporal order, but this information is lost in the final stage, where temporal averaging is applied.
We argue that the value of the lost information increases with the length of the video, and that this information can be leveraged by switching to a different pooling function.
%  is still valuable information in the temporal arrangement of the features that can be extracted with a suitable pooling function and that the amount of information lost by order-agnostic pooling increases with the length of the videos.

\paragraph{Temporal transformer.}

We propose to tackle this issue by replacing average pooling in time $\mathcal{P}_t$ in~\cref{e:decomp} with a transformer $\mathcal{P}_\text{transf}$.
Transformers~\citep{vaswani2017attention} have been shown effective for representing sequential inputs in the NLP domain~\citep{bert18, raffel2019exploring, lewis2019bart, radford2019language}.
After spatial averaging, the output $\bh=\mathcal{P}_s(\Psi(\tilde \bv)) \in \mathbb{R}^{D\times T_1}$ of the network has one feature vector per time step, and is thus amenable to processing by a transformer.
The feature $\bh$, which differs in latent time-dimension size from its uncropped variant can be seen as masking the transformer's attention.
Masking attention has been used in transformer encoder-decoder training to prevent the model from cheating~\citep{devlin18bert:} and encourage it to leverage information from the context.
%
We use a shallow and light-weight transformer on top of our feature cropping procedure, which we show to be sufficient to reap the benefit of better temporal modelling incurring only a very small computational cost.
We use 2-layers and 4 self-attention heads and provide further details on the transformer architecture in the Appendix.
%In practice, we use , with Layer-normalization~\citep{ba16layer}.
%stack of transformers with 4 self-attention heads upon the video backbone.,
% $
% \mathcal{P}_\text{transf}
% (\bh) = 
% (T_2 \circ T_1(\bh))[0]
% $,
% where
% $
% T(\bh)
% =
% \text{LN}(\text{FFN}(M(\bh))+M(\bh)) 
% $ and $M(\bh) = \text{LN}(\bh+\text{MHA}(\bh))$
% is the transformer with multi-head self-attention (MHA), layer-normalization~\citep{ba2016layer} (LN), and feed-forward network (FFN).
% We provide further details about transformer architecture in the Appendix.

% While is hard to quantify how much information is lost by the temporal pooling function of common models, the penultimate feature dimensions do scale proportionally with the input temporal dimension.
% The transformer pooling is therefore a viable strategy in particular for longer videos, which allow for better modelling of the order.

\subsection{Overall loss}
% We are now ready to put the various components of our model together.
Our combined model, \textbf{\methodname}, better learns space-time invariances and relationships by cropping in space-time and leveraging  temporal attention with a transformer.
For training, we sample $N$ videos in a batch and, for each of them, compute two `large' visual crops in RGB space, $2(n+m)$ small and medium feature crops (\cref{s:featurecrop}), and an audio augmentation $a$.
With those, the overall objective is obtained by summing the within-modality loss $L_{vv}$ from~\cref{e:lossvisual} to the cross modality losses:
\begin{align}
L
& =
\lambda_{vv} L_{vv} + \lambda_{va} L_{va}, \label{loss:total}
\end{align}
where $L_{va} {=} 
\mathcal{L}(v_{L_1}, a)
+
\mathcal{L}(v_{L_2}, a)
+
\mathcal{L}(a,v_{L_1})
+
\mathcal{L}(a,v_{L_2})
$.




==> STiCa (ICCV 2021)/4_experiments.tex <==
\section{Experiments}\label{s:experiments}

\input{tabs/ABL_table}

We first describe the datasets (\cref{s:datasets}) and implementation details (\cref{s:impl_details}) for pretraining.
In \cref{s:downstream}, we describe the downstream tasks for evaluating the representation obtained from self-supervised learning.
In~\cref{s:ablation}, we ablate the various components of our method, and the importance of temporal context and multi-modality in \cref{s:findings}.
Lastly, in \cref{s:sota}, we compare with prior work in video and multi-modal representation learning.

\paragraph{Data.\label{s:datasets}}

We pretrain on the Kinetics-400 dataset~\citep{kinetics}, which contains about 230K training videos and 13K validation videos belonging to 400 action classes.
This dataset is the ``ImageNet'' for video representation learning due to its moderate size and being public, allowing for broad access and comparability.
After pretraining, we evaluate using video action retrieval and action recognition on HMDB-51~\citep{HMDB51} and UCF-101~\citep{UCF101}.
HMDB-51~\citep{HMDB51} consists of 7K video clips spanning 51 different human activities.
HMDB-51 has three train/test splits of size 5K/2K respectively.
UCF-101~\citep{UCF101} contains 13K videos from 101 human action classes, and has three train/test splits of size 11K/2K respectively.

\paragraph{Implementation details.\label{s:impl_details}}

Following~\citep{Patrick2020MultimodalSF}, we use the R(2+1)-18~\citep{Tran18} network as visual encoder and ResNet~\citep{he16resnet} with 9 layers as audio encoder. 
We train for $100$ epochs and use $30$ frames with temporal stride of 1 at sampling rate of 30fps at spatial resolution of $112\times112$ as input.
In our ablations, we evaluate the learned representation by finetuning the visual encoder on fold 1 of the HMDB-51~\citep{HMDB51} action recognition dataset.
Further implementation details are given in the Appendix.

% We use either average pooling or a transformer as pooling function for the visual encoder, but always use average pooling for the audio encoder. The transformer's layers dimensionality are set to 512-D.
% Both encoders produce a fixed-dimensional representation vectors after temporal aggregation (512-D).
% Both vectors are then passed through two fully-connected layers with intermediate size of $512$ to produce 256-D embedding vectors $\bz$ as in~\citep{Patrick2020MultimodalSF}.
% We use these embeddings in our loss eq.~\eqref{loss:total} and train our model for $100$ epochs.
% For the visual component of the video, we use a $30$ frame RGB clip as input, at $30$ fps covering 1 second.
% The video clip has a spatial resolution of $112 \! \times \!112$ pixels.
% For input data augmentation, we apply random crops, horizontal flips, Gaussian blur and color jittering, all clip-wise consistent, following the protocol of SimCLR~\citep{Chen2020ASF}, and we ablate multiple settings for spatial and temporal feature cropping sizes.
% For the audio input, we extract a $1$-second log-mel spectrogram of dimension $257\times 199$ starting at the same time as the visual component.
% We also apply volume jittering to increase the robustness of our audio features.
% We optimize this model using SGD with momentum $0.9$, weight decay $10^{-5}$ and learning rate $0.64$, with a warm-up period of $10$ epochs.
% For NCE contrastive learning, the temperature $\tau$ is set as $0.1$ for cross-modal loss, and $0.5$ for the within-modal loss.
% We use a mini-batch size of $8$ on each of our $64$ GPUs giving an effective batch size of $512$ for distributed training.
% In our ablations, we evaluate the learned representation by finetuning the visual encoder on fold 1 of the HMDB-51~\citep{HMDB51} action recognition dataset.

\subsection{Downstream tasks\label{s:downstream}}

% \paragraph{Linear Evaluation.}
% For linear evaluation, we closely follow the protocol of CVLR~\citep{Qian2020SpatiotemporalCV}.
% We fix the weights of our video backbone, and add a linear layer of dimension $400$.
% We train this linear layer for $100$ epochs with SGD, momentum $0.9$ and learning rate $32$.
% We warm-up the learning rate for $5$ epochs, and decay the learning rate at epochs $60$ and $90$ by $0.1$.

\paragraph{Video action retrieval.}

For video retrieval, we follow the standard protocol described in~\citep{clip_order}.
We use the split 1 of UCF-101, and additionally HMDB-51.
We uniformly sample $10$ clips per video, max pool and then average the features after the last residual block for each clip per video.
We use these averaged features from the validation set to query the videos in the training set.
If the class of a retrieved video matches the class of query video, we count it as a match.
We measure recall at $k{=}1,5,20$.

\paragraph{Video action recognition.}

As is standard in the literature, we evaluate our pretrained representations by finetuning our visual backbone on the video action recognition task on HMDB-51 and UCF-101 datasets.
We closely follow the finetuning schedule of GDT~\citep{Patrick2020MultimodalSF}.
During finetuning, we use SGD with initial learning rate $0.0025$, which we gradually warm up to $0.02$ in the first $2$ epochs
The weight decay is set to $0.005$ and momentum to $0.9$.
We use a mini-batch size of $32$ and train for $12$ epochs with the learning rate multiplied by $0.05$ at $6$ and $10$ epochs.
For training, we randomly sample $1$s clips per video, and during evaluation, we uniformly sample $10$ clips from each video and apply 3-crop evaluation as in~\citep{slowfast}.

\subsection{Comparison experiments and ablations\label{s:ablation}}

\paragraph{Cropping augmentation.}

In~\Cref{tab:ablation:spatial_crop}, we ablate the importance of spatial augmentation in learning video representations.
We compare our proposed Feature Crop augmentation, $C_{\bar B}$, to the recently proposed Multi-Crop augmentation strategy~\citep{caron2020swav} and other baseline approaches.
Multi-Crop has proven to be effective in image self-supervised learning because it forces the model to learn local-to-global associations, by explicitly enforcing invariance between features of large-crops and those of multiple small crops.
While effective, it can be particularly computationally intensive, which, with our hardware, limits its use to only two large crops and one small crop when applied to video representation learning.
Our proposed Feature Crop is not only more efficient, but outperforms Multi-Crop by $1.1\%$ when the learned representations is applied to action classification in HMDB-51.
By cropping in feature space, we achieve a similar effect but can increase the number of small crops from 1 to 6 without increasing compute time.



\paragraph{Feature crop parameters.}

In~\Cref{tab:ablation:feature_crop}, we study the parameters of our Feature Cropping approach.
We find that even our basic variant, which does one medium $6 \! \times \!6$ crop and two $4\! \times \! 4$ small crops (by cropping a $7\! \times \!7$ tensor) increases performance by nearly $6\%$, which is a relative improvement of more than $10\%$.
If we further increase the number of crops in time and space, the performance increases from $59.9\%$ to $60.4\%$.

\paragraph{Pooling Function.}

In~\Cref{tab:ablation:pooling}, we test temporal aggregation.
We find that using a shallow transformer significantly outperforms simple average pooling by more than $5\%$; however, transformer pooling must be used both for pre-training the representation and for finetuning it on the target dataset.

\paragraph{Transformer architecture.}

In~\Cref{tab:ablation:num_layers_heads}, we test variants of the transformer architecture, including ablating iit altogether.
% We find that temporal modelling as measured by downstream performance first increases with depth, but starts decreasing when using 4 layers, likely due to optimization difficulties of deeper transformers with SGD.
We find that temporal modelling as measured by downstream performance peaks at two layers, likely due to optimization difficulties of deeper transformers with SGD\@.
We also compare to a model with approximately the same number of parameters as our 2-layer transformer (achieved by increasing the networks' last block's hidden dimension to $640$).
We find that the transformer still yields gains of $3\%$, indicating that it not the number of parameters but the modelling of time that is crucial for strong performance.

\paragraph{Combining Feature Crops and Transformer Pooling.}

In~\Cref{tab:ablation:cumul_gains}, we show that combining Feature Crops in space and time, and then adding transformer pooling yield additive gains, with the best result obtained by combining all effects (which corresponds to \textbf{\methodname}).
This shows that space-time augmentations and transformer pooling are complementary.
% As shown in the last row, \textbf{\methodname}, \ie~doing Feature Crops in space and time, as well as temporal modelling with a transformer outperforms each contribution applied separately.

\paragraph{Cropping efficiency.}

In~\Cref{tab:ablation:cropvstime}, we compare training times (normalized to GPUs$\times$hours) for Kinetics-400 epochs for the various spatial crops considered.
We make two observations: First, the compute cost of RGB crops scales proportionally to their number because a full forward pass is required for each crop. Second, using a larger number of RGB crops eventually requires to decrease the batch size, which increases significantly the training time.
In contrast, the cost of Feature Crop remains roughly constant no matter the number of crops.

\begin{table}
\footnotesize
\centering
\makebox[0pt][c]{\parbox{0.48\textwidth}{%
\begin{minipage}[b]{0.48\hsize}\centering
    \input{tabs/abl_num_frames}
    \vspace{-1em}
\end{minipage}
\hfill
\begin{minipage}[b]{0.42\hsize}\centering
    \input{tabs/abl_loss}
    \vspace{-1em}
\end{minipage}
}}
\end{table}

\subsection{Temporal Context and Multi-modality\label{s:findings}}

\paragraph{Length of temporal context.}

In~\Cref{tab:ablation:transformer}, we show the importance of leveraging longer context to improve video self-supervised representation learning.
Similar to the supervised regime~\citep{varol17, XiaolongWang18}, we observe improved accuracy as we increase the number of frames used during pretraining and fine-tuning.
More importantly, the transformer pooling layer is better able to exploit this additional context, outperforming average pooling by over $4\%$ for all frame lengths.
Notably, there is a drop in performance when using GAP for extremely long contexts (90 frames).

\input{tabs/full_transfer}

\paragraph{Loss.}

Lastly, in~\Cref{tab:ablation:loss}, we study the effect of combining multi-modal learning signals with our contributions.
In the first row, we have the baseline of naively extending SimCLR~\citep{Chen2020ASF} to the video domain, by learning invariances to spatial augmentations of two large-crops.
Compared to this, the cross-modal baseline (row 2) already achieves gains of more than $10\%$.
% However, we see that within-modal learning can actually work quite well if our feature-crop augmentation is used as additional augmentation.
% By using feature-crops of size $2\!\times \!6^2 \!+ \!4\!\times \!4^2$ for spatial and  $2\!\times \!3 \! + \! 1\!\times \!2$ for temporal crops, we find the performance is $ww$, $ww-43.3\%$ better than row 1.
% Finally, we find that the cross-modal signal is complementary to our spatial invariance inducing feature-crops with a performance of $XXXX$.
While adding a within-modal invariance adds another 4.6\%, we find that the best performance is obtained with our feature crops, adding another 1.7\% in performance and showing its unique potential to supplement cross-modal signals.
%feature-crops of size $2\!\times \!6^2 \!+ \!4\!\times \!4^2$ for spatial and  $2\!\times \!3 \! + \! 1\!\times \!2$ for temporal crops as augmentation for video-only loss with a cross-modal loss, we see performance improvements of $6\%$ over just learning cross-modal signals.

\subsection{Comparison with the state of the art\label{s:sota}}

\paragraph{Video Action Recognition.}

In~\Cref{tab:sota_full_transfer}, we evaluate our pretraining approach on the standard HMDB-51 and UCF-101 action recognition benchmarks after pretraining on the Kinetics-400 dataset. %, comparing to the state-of-the-art.
Firstly, we find our model outperforming the similar NCE-based GDT~\citep{Patrick2020MultimodalSF} model by $7.0\%$ and $3.8\%$ on HMDB-51 and UCF-101.
% We further significantly outperform current state-of-the art methods CoCLR~\citep{Han2020SelfsupervisedCF} and concurrent CVLR~\citep{Qian2020SpatiotemporalCV} by $xx \%$ and $xx \%$ on HMDB-51 and UCF-101.
We further significantly outperform the current state-of-the art methods \mbox{CoCLR}~\citep{Han2020SelfsupervisedCF} by $4.1\%$ and $2.5\%$ and CVLR~\citep{Qian2020SpatiotemporalCV} by $2.6\%$ and $1.0\%$ on HMDB-51 and UCF-101, respectively.
Even more impressively, our approach is able to out-perform most prior works that use AudioSet~\citep{AudioSet} pre-training, which is around 10$\times$ larger than Kinetics-400.
This shows how effective and data-efficient our approach is, significantly closing the gap to supervised learning.

\paragraph{Video Action Retrieval.}

Lastly, we directly evaluate the transfer-ability of our pretrained representations on action retrieval on UCF-101 and HMDB-51.
Similarly to full fine-tuning setting, we outperform all prior works.

%\input{tabs/sota_linear}
\input{tabs/sota_retrieval}


==> STiCa (ICCV 2021)/6_conclusion.tex <==
\section{Conclusion}
%In this paper, we show that, in fact, further significant gains can be obtained by better representing time as well as spatial information.
%For time, we show that the use of transformers, as opposed to naive average pooling, improves performance significantly, especially when it is applied to longer video clips.
%For space, we show that spatial augmentations, which so far have achieved little improvements in multi-modal self-supervised learning, can indeed bring significant benefits provided that the right augmentation statistics are selected.
% Augmentations are of tremendous importance for self-supervised representation learning.
% In this work, We address two shortcomings of current methods for video data, nameley insufficient spatial invariance signals (especially compared to images) and insufficient modelling of time (unique to videos).
We have address two shortcomings of current self-supervised video representation learning: insufficient spatial invariance, especially compared to the image domain, and inadequate modelling of time.
We have introduced \methodname, improving spatial invariance at very little cost by implementing cropping in feature space, and improving modelling of time via a shallow transformer.
%  propose a new efficient learning method, STACr, that can cheaply generate a multitude of crops and better model time in feature space.
%Used with a noise-contrastrative task, we study the effects of both of our contributions in detail and demonstrate significant gains w.r.t.~the state-of-the-art.
Our method brings self-supervised video representation learning one step closer to the supervised case, providing significant gains w.r.t.~the state-of-the-art.

%We study the effects of both of our contributions in detail and demonstrate significant gains w.r.t.~the state-of-the-art by better exploiting spatial and temporal infomation for self-supervised video representation learning.
% We belief this work bring video representation learning closer to modelling 
% We believe the contributions in this paper bring self-supervised learning for video closer to their supervised counterparts and could 

% We have addressed two shortcomings of current self-supervised representation learning methods for video data,
% the lack of sufficient spatial augmentation and the suboptimal modelling of time. 
% By introducing respectively Feature Crops and the use of Transformer pooling functions for time,  we have demonstrated significant improvements w.r.t.~the state-of-the-art.


==> STiCa (ICCV 2021)/figs/fig-method.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.9\linewidth]{figs/stica_final.pdf}
\vspace{-0.1in}
\caption{\textbf{Approach Overview.} We present a self-supervised approach that learns video representations without labels. \textbf{(Top)} Prior work in video representation learning did not capture spatial invariances, as taking many crops of the input (at varying locations and scales), quickly gets expensive in both compute and memory.
% Furthermore, the features are aggregated by global spatial- and temporal-pooling, which does not fully leverage the signal left in the latent temporal dimension.
\textbf{(Bottom)} The proposed method generates a large variety of views from only two RGB-crops by cropping in latent space and is particularly tailored to  self-supervised contrastive learning.
The latent crops are essentially masked features, which are 
then further processed by a light-weight temporal transformer. Compared to global pooling, this allows our method to further capture the rich temporal signal.
}
\label{fig:short}
\vspace{-1.0em}
\end{figure*}

==> STiCa (ICCV 2021)/figs/fig-splash.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.99\linewidth]{figs/splash_final.pdf}
\vspace{-1em}
\end{center}
   \caption{\textbf{HMDB-51 accuracy vs epoch.} 
   Our method, \textbf{\methodname}, combines space-time crops in feature space with self-attention of time in latent space. 
   This yields significant benefits not only in performance but also in speed compared to cropping in input space using \textit{two RGB crops}, or simply using the \textit{default} cross-modal only loss. 
%   In addition, we introduce better modelling of the latent temporal dimension with transformers, adding further gains.
   Compared to recent state-of-the-art cross-modal self-supervised learning methods 
   (XDC~\cite{alwassel2019self}, GDT~\cite{Patrick2020MultimodalSF}, AVID-CMA~\cite{morgado2020avid}, SeLaVi~\cite{asano2020labelling}) pre-trained on Kinetics-400~\cite{kinetics}
   \methodname{} is able to achieve significantly better results in fewer epochs. 
   \label{fig:splash}
   }
\end{figure}


==> STiCa (ICCV 2021)/tabs/ABL_table.tex <==
\begin{table*}[tb]
\footnotesize
\caption{\textbf{Comparison experiments and ablations.} We compare key parameters and settings of our proposed method. We report results model performance at epoch 100 and with 30 frames and without transformer unless noted otherwise.
}\label{tab:ablation}
\setlength{\tabcolsep}{3pt}
	\begin{subtable}[t]{.58\linewidth}\centering
		{\input{tabs/_abl_1a}}	
	\end{subtable}
	\hfill
	\begin{subtable}[t]{.39\linewidth}\centering
		{\input{tabs/_abl_1b}}	
	\end{subtable}
	\\
% 	\vspace{1em}
	\begin{subtable}[t]{.29\linewidth}\centering
	    {\input{tabs/_abl_1c}}	
	\end{subtable}
	\hfill
	\begin{subtable}[t]{.33\linewidth}\centering
		{\input{tabs/_abl_1d}}	
	\end{subtable}
	\hfill
	\begin{subtable}[t]{.31\linewidth}\centering
		{\input{tabs/_abl_1e}}	
	\end{subtable} \\ 
% 	\vspace{-1em}
	\begin{subtable}[t]{.98\linewidth}\centering
		{\input{tabs/_abl_1f}}	
	\end{subtable}
% 	\\
% 	\begin{subtable}[b]{.45\linewidth}\centering
% 		{\input{tabs/abl_num_frames}}	
% 	\end{subtable}
% 	\begin{subtable}[b]{.34\linewidth}\centering
% 		{\input{tabs/abl_cumulative_gains}}	
% 	\end{subtable}
\vspace{-2.0em}
\end{table*}

==> STiCa (ICCV 2021)/tabs/_abl_1a.tex <==
% \begin{table}
% \begin{center}
\footnotesize
\begin{tabular}{llcc}
\toprule
Cropping-strategy                    & Resolution                               & GPU-h/epoch & Acc. \\
\midrule
Default                              & $1\!\times \!112^2$                      & $17.3$      & $54.0$ \\
Two RGB Crops                        & $2\!\times \!112^2$                      & $29.3$      & $58.6$ \\
Multi RGB Crops~\cite{caron2020swav} & $2\!\times \!112^2$ + $1\!\times \!96^2$ & $46.7$      & $59.3$ \\
Ours (Feature Crop)                  & $2\!\times \!112^2$  + latent            & $29.3$      & $\bf{60.4}$ \\
\bottomrule
\end{tabular}
\vspace{0.5em}
\caption{\textbf{Cropping} yields benefits but requires more compute.
Our feature crops are efficient \textit{and} outperform~\cite{caron2020swav}.
Note that all models are trained for 100 epochs.%
\label{tab:ablation:spatial_crop}}
\vspace{-1em}

==> STiCa (ICCV 2021)/tabs/_abl_1b.tex <==
% \begin{table}
% \begin{center}
\begin{tabular}{c cc cc}
\toprule
\multicolumn{2}{c}{\underline{$l$-Spatial size}} & \multicolumn{2}{c}{\underline{$l$-Temporal size}} & Acc. \\
$M$ & $S$ & $M$ & $S$ \\
% \hline
\midrule
$1\!\times7^2$        &                       & $1\!\times4$        &                   & $54.0$\\
$1\!\times \!6^2$  & $\! 2\!\times \!4^2$  & $1\!\times4$         &                  & $59.9$ \\ 
% $2\!\times \!6^2$   + $4\!\times \!4^2$     & $1\!\times4$                            & $59.5$ \\ 
$1\!\times \!6^2$  & $\!2\!\times \!4^2$   & $2\!\times \!3$        & $\! 1\!\times \!2$ & $58.4$ \\
$2\!\times \!6^2$  & $\!4\!\times \!4^2$   & $2\!\times \!3$        & $\! 1\!\times \!2$ & $\bf{60.4}$ \\
\bottomrule
\end{tabular}
% \end{center}
\caption{\textbf{Feature crops.} Heavier augmentations in latent~($l$) space and time lead to better representations.\label{tab:ablation:feature_crop}}
% \end{table}

==> STiCa (ICCV 2021)/tabs/_abl_1c.tex <==
\begin{tabular}{llc}
\toprule
Pretraining  & Finetuning & Acc \\
\midrule
$\mathcal{P}_t$             & $\mathcal{P}_t$             & $54.0$ \\
$\mathcal{P}_t$             & $\mathcal{P}_\text{transf}$ & $54.6$ \\
$\mathcal{P}_\text{transf}$ & $\mathcal{P}_t$             & $52.1$ \\
$\mathcal{P}_\text{transf}$ & $\mathcal{P}_\text{transf}$ & $\bf{60.3}$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Pooling.} Compared to Average-Pooling ($\mathcal{P}_t$), Transformer-based pooling ($\mathcal{P}_\text{transf}$) gives stronger performance.\label{tab:ablation:pooling}}

==> STiCa (ICCV 2021)/tabs/_abl_1d.tex <==
% \begin{table}
\begin{center}
\begin{tabular}{ccccc}
\toprule
Transf.? & Layers & Params & GFLOPS & Acc. \\
\midrule
\xmark & $0$ & $37.2$M & $77.7$ & $54.0$ \\
\xmark & $0$ & $42.8$M & $80.0$ & $57.3$ \\
%$1$ & $39.8$M & $77.7$ & $xx$ \\
\cmark & $2$ & $42.4$M & $77.8$ & $\bf{60.3}$ \\
\cmark & $4$ & $47.7$M & $77.8$ & $58.3$ \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-1em}
\caption{\textbf{Architecture.} Using up to two transformer layers gives gains, not due to more trainable parameters.\label{tab:ablation:num_layers_heads}}
% \end{table}


==> STiCa (ICCV 2021)/tabs/_abl_1e.tex <==
% \begin{table}
% \begin{center}
\begin{tabular}{cccc}
\toprule
$C_\mathrm{space}$ &  $C_\mathrm{time}$  & T?  & Acc. \\
\midrule
{\color{gray}\xmark} & {\color{gray}\xmark} & {\color{gray}\xmark} & $54.0$ \\
% None                      & None & \checkmark & $58.9$ \\ 
% $2\!\times \!6^2$ + $4\!\times \!4^2$  & None & \xmark & $~60.0tbd$ \\ 
% $2\!\times \!6^2$ + $4\!\times \!4^2$  & None & \xmark & $59.9$ \\
% $2\!\times \!6^2$ + $4\!\times \!4^2$  & $1\!\times \!3$ + $2 \! \times \!2$ & \xmark & Yuki \\
% $2\!\times \!6^2$ + $4\!\times \!4^2$  & $1\!\times \!3$ + $2 \! \times \!2$ & \cmark & Bernie\\
\cmark  & {\color{gray}\xmark} & {\color{gray}\xmark} & $59.9$ \\
\cmark  & \cmark & {\color{gray}\xmark} & $60.4$ \\
\cmark  & \cmark & \cmark & $\bf{62.0}$\\
\bottomrule
\end{tabular} 
% \vspace{-1em}
\caption{\textbf{Combined gains.} Feature crop in space $C_\mathrm{space}$ and time $C_\mathrm{time}$ and transformer pooling (T) add cumulative benefits. \label{tab:ablation:cumul_gains}}
% \vspace{-1em}
% \end{table}

==> STiCa (ICCV 2021)/tabs/_abl_1f.tex <==
% \begin{table*}[tb]
    % \centering
    % \footnotesize
    % \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c ccc | ccc | cc}
        \toprule
        Method &  \multicolumn{3}{c}{\textbf{RGB-Crops}} & \multicolumn{3}{c}{\textbf{Multi-scale RGB-Crops}} & \multicolumn{2}{c}{\textbf{Feature Crops}}\\
        & 1x & 2x & 4x{\color{red}$^*$}  & 2x112 + 1x96 & 2x112 + 2x96 & 2x112 + 6x96{\color{red}$^*$} & (1x7, 1x4) & (2x6 + 4x4, 2x3 + 1x2) \\
        \midrule
        GPU-h/epoch & 17.3 & 29.3 & 60.0 & 46.7 & 53.3 & 100.7 & 29.3 & 30.0  \\
        % GPU-mem/BS & xx & xx & {\color{red} xx} & xx & xx & {\color{red}xx.x} & xx & xx  \\
        \bottomrule
    \end{tabular} 
% \vspace{-0.5em}
\caption{\textbf{Speed.} Input-crops are slow: {\color{red}$*$} methods require reducing batch sizes (see Appendix) as activations do not fit on GPU. \label{tab:ablation:cropvstime}}
% \end{table*}


==> STiCa (ICCV 2021)/tabs/abl_loss.tex <==
% \begin{table}
% \setlength{\tabcolsep}{1pt}
% \begin{wraptable}{r}{3.5cm}
% \centering
%
% \footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{cccc}
\toprule
$\lambda_{va}$ &  $\lambda_{vv}$  & F. Crop?  & Acc. \\
\midrule
0    & 1   & No  & $43.3$ \\
1    & 0   & No  & $54.0$ \\
0.5  & 0.5 & No  & $58.6$ \\
0.5  & 0.5 & Yes & $\bf{60.3}$\\
\bottomrule
\end{tabular} 
\vspace{-0.5em}
\caption{\textbf{Loss.} Combining within-modal and cross-modal loss with Feature-crops is key. \label{tab:ablation:loss}}
% \end{table}
% \vspace{-1em}


==> STiCa (ICCV 2021)/tabs/abl_num_frames.tex <==
% \begin{wraptable}{r}{3.5cm}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c c c c c}
\toprule
\multicolumn{2}{c}{\underline{{Frames}}} &   & \multicolumn{2}{c}{\underline{{Accuracy}}} \\
% \cmidrule{1-2} \cmidrule{4-5}
Pretrain & Finetune & & GAP    & Transf.       \\
\midrule
30       & 30       & & $54.0$ & $\bf{60.3}$  \\
60       & 60       & & $62.4$ & $\bf{66.1}$ \\
90       & 90       & & $58.0$ & $\bf{66.9}$\\
\bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{\textbf{Temporal context.} We report results with different number of frames on finetuning accuracy.\label{tab:ablation:transformer}}


==> STiCa (ICCV 2021)/tabs/abl_transformer_pos.tex <==
\begin{table}
\begin{center}

\begin{tabular}{cc}
\toprule
Pos Encoding.  & Acc. \\
\midrule
\xmark  & $62.7$ \\
\cmark  & $62.1$\\
\bottomrule
\end{tabular} 
\end{center} 
\caption{\textbf{Transformer Positional Encoding.} Positional encoding makes little difference in final performance. \label{tab:ablation:pos_encoding}}
\end{table}

==> STiCa (ICCV 2021)/tabs/appx_sota_audio.tex <==
\begin{table}
\begin{tabular}{l l cc} 
\toprule
\textbf{Method}                         & \textbf{Pretraining} &\multicolumn{2}{c}{\underline{\textbf{Acc\%}}} \\
                                        &           & DCASE  & ESC50 \\
\midrule
Autoencoder \cite{aytar2016soundnet}    & -    & -        &   39.9        \\
Random Forest \cite{esc50}              & -    & -        &   44.3        \\
Piczak ConvNet \cite{Piczak2015}        & -    & -        &   64.5        \\
RNH \cite{rnh2013}                      & -    & 72       &   -           \\
Ensemble \cite{stowell2015}             & -    & 77       &   -           \\
ConvRBM \cite{sailor2017}               & -    & -        & 86.5          \\
\midrule
AVTS \cite{avts}                        & K400   & 91       & 76.7          \\
XDC \cite{alwassel2019self}             & K400   & --       & 78.0          \\
AVID \cite{morgado2020avid}             & K400   & \ul{93}  & 79.1         \\
ACC \cite{ma2020learning}               & K400   & --       & \ul{79.2}       \\
\midrule
\textbf{Ours: \methodname}                    & K400  & \bf{94}   &   \bf{81.1}           \\
\midrule
SoundNet \cite{aytar2016soundnet}       & SNet  & 88        & 74.2          \\
L3-Net \cite{Arandjelovic17}            & SNet  & 93        & 79.3          \\
AVTS \cite{avts}                        & SNet  & 94        & 82.3          \\
DMC \cite{hu2018deep}                   & SNet & --         & 82.6          \\
\midrule
AVTS \cite{avts}                        & AS   & 93        & 80.6          \\
XDC \cite{alwassel2019self}             & AS   & --        & 85.8          \\
MMV \cite{alayrac2020selfsupervised}    & AS   & --        & 86.1       \\
AVID \cite{morgado2020avid}             & AS   & \ul{96}   & \ul{89.2}      \\
GDT \cite{Patrick2020MultimodalSF}      & AS   & \bf{98}   & 88.5       \\
ACC \cite{ma2020learning}               & AS   & --        & \bf{90.8}       \\
\midrule
Human \cite{esc50}                      & -- & --      & 81.3 \\
\bottomrule
\end{tabular} 
\caption{\textbf{Audio classification.} 
Downstream task accuracies on standard audio classification benchmarks on DCASE2014 and ESC50. Dataset abbreviations
  \textbf{\ul{A}}udio\textbf{\ul{S}}et, 
  \textbf{\ul{K}}inetics\textbf{\ul{400}},
  \textbf{\ul{S}}ound\textbf{\ul{Net}},
  \label{tab:audio}}
\end{table}

==> STiCa (ICCV 2021)/tabs/full_transfer.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\footnotesize
\begin{center}
\begin{tabular}{l l l  c c }
\toprule
	\textbf{Method}                              & \textbf{Architecture} & \textbf{Dataset} &
	\multicolumn{2}{c}{\textbf{Top-1 Acc\%}} \\
				                               &  &      & HMDB & UCF       \\
\midrule
	Supervised                                & R(2+1)D-18  & K-400 & 70.4  & 95.0 \\
\midrule
% 	RotNet3D~\cite{jing2018self}              & R3D-18      & K-400 & 33.7 & 62.9  \\
% 	DPC~\cite{han2019video}                   & R3D-34      & K-400 & 35.7 & 75.7  \\
% 	CBT~\cite{sun2019contrastive}             & S3D+BERT    & K-400 & 44.6 & 79.5  \\
% 	PacePred~\cite{Wang2020SelfsupervisedVR}  & R(2+1)D-18  & K-400 & 36.6 & 77.1  \\
% 	SpeedNet~\cite{benaim2020speednet}        & S3D-G       & K-400 & 48.8 & 81.1  \\
%	Multisensory~\cite{owens2018audio}        & R3D-18      & K-400 & -    & 82.1  \\
	SeLaVi~\cite{asano2020labelling}          & R(2+1)D-18  & K-400 & 47.1 & 83.1  \\
	TempTrans~\cite{Jenni2020VideoRL}     & R3D-18      & K-400 & 49.8 & 79.3  \\
	PEMT~\cite{lee2021parameter} & SlowFast & K-400 & - & 85.2 \\
	XDC~\cite{alwassel2019self}               & R(2+1)D-18  & K-400 & 52.6 & 86.2  \\
	MemDPC~\cite{Han2020MemoryaugmentedDP}    & R-2D3D      & K-400 & 54.5 & 86.1 \\
	AVSF~\cite{xiao2020audiovisual}    & AVSF  & K-400 & 54.6 & 87.0  \\
	AVTS~\cite{avts}                          & MC3-18      & K-400 & 56.9 & 85.8  \\
	CPD~\cite{li2020learning}                 & R3D-50      & K-400 & 57.7 & 88.7  \\
	AVID~\cite{morgado2020avid}               & R(2+1)D-18  & K-400 & 60.8 & 87.5  \\
	GDT~\cite{Patrick2020MultimodalSF}        & R(2+1)D-18  & K-400 & 60.0 & 89.3  \\
	ACC~\cite{ma2020learning}                 & R3D-18      & K-400 & 61.8 & 90.2  \\
	GLCM~\cite{ma2021contrastive}              & R3D-18      & K-400 & 61.9 & 91.2  \\
	CoCLR~\cite{Han2020SelfsupervisedCF}      & S3D         & K-400 & 62.9 & 90.6  \\
	CVLR~\cite{Qian2020SpatiotemporalCV}\footnote{Concurrent work.}      & R3D-50      & K-400 & 66.7 & 92.2 \\ % old numbers: & K-400 & 65.4 & 92.1  \\
\midrule
	\bf{Ours: \methodname}                                 & R(2+1)D-18  & K-400 & \bf{67.0} &\bf{93.1}  \\
\midrule
\midrule
\color{gray}
%    L3-Net~\cite{Arandjelovic17}             & VGG-16     & AS      & 40.2      & 72.3\\
    SeLaVi~\cite{asano2020labelling}         & R(2+1)D-18 & VGGS    & 53.1      & 87.7\\
    Speech2Act~\cite{nagrani2020}            & S3D-G      & Movie   & 58.1      & -- \\
    DynamoNet~\cite{Diba_2019}               & ResNext101 & Y8M     & 58.6      & 87.3\\
	MIL-NCE~\cite{miech2019endtoend}         & S3D        & HT      & 61.0      & 91.3\\
    AVTS~\cite{avts}                         & MC3-18     & AS      & 61.6      & 89.0\\
    %XDC~\cite{alwassel2019self}              & R(2+1)D-18 & AS      & 63.7      & 93.0\\
	AVID~\cite{morgado2020avid}              & R(2+1)D-18 & AS      & 64.7      & 91.5\\
	Textual~\cite{Stroud2020LearningVR}      & S3D-G      & WVT-70M & 65.3      & 90.3 \\
	GDT~\cite{Patrick2020MultimodalSF}       & R(2+1)D-18 & AS      & 66.1      & 92.5\\
	\cdashlinelr{1-1}
	ACC~\cite{ma2020learning}                & R(2+1)D-18 & AS      & 67.2      & 93.5  \\
	ELo~\cite{piergiovanni2020evolving}      & R(2+1)D-50 & Y2M     & 67.4      & 93.8\\
	XDC~\cite{alwassel2019self}              & R(2+1)D-18 & IG65M   & 68.9      & \bf{95.5}\\
	% MMV~\cite{alayrac2020selfsupervised}     & R(2+1)D-18 & AS      & 70.1      & 91.5  \\
	GDT~\cite{Patrick2020MultimodalSF}       & R(2+1)D-18 & IG65M   & {72.8}      & 95.2\\
	MMV~\cite{alayrac2020selfsupervised}     & TSM-50x2   & AS+HT   & \bf{75.0} & 95.2\\
% \midrule
% 	\bf{Ours}                                 & R(2+1)D-18  & K-400 & 66.5 & 92.2  \\ % should be audioset right?
\bottomrule
\end{tabular}
\end{center}
\vspace{-1.5em}
\caption{\textbf{Comparison to SoTA for action recognition}. Dashed line indicates position of our Kinetics-400 model in comparison to models trained with many more videos. We follow standard evaluation protocol across 3-folds. For linear evaluation results see~\cref{tab:sota_linear}. \label{tab:sota_full_transfer}}
% \vspace{-1.0em}
\end{table}

==> STiCa (ICCV 2021)/tabs/sota_linear.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[tb]
\begin{center}
\begin{tabular}{l l l c c }
\toprule
	\textbf{Method}                              & \textbf{Architecture} & \textbf{Dataset} &
	\multicolumn{2}{c}{\textbf{Top-1 Acc\%}} \\
				                              &    &   & HMDB & UCF       \\
\midrule
	RotNet3D~\cite{jing2018self}              & S3D         & K600 & 24.8 & 47.7  \\
	CBT~\cite{sun2019contrastive}             & S3D+BERT    & K600 & 29.5 & 54.0  \\
	MemDPC~\cite{Han2020MemoryaugmentedDP}    & R-2D3D      & K400 & 30.5 & 54.1  \\
	AVSF~\cite{xiao2020audiovisual}           & AVSF        & K400 & 44.1 & 77.4  \\
	CoCLR~\cite{Han2020SelfsupervisedCF}      & S3D         & K400 & 46.1 & 74.5  \\
	\midrule
    \bf{Ours:  \methodname}                         & R(2+1)D-18  & K400  & \bf{48.2} & \bf{77.0}  \\
    \midrule
	MIL-NCE~\cite{miech2019endtoend}          & S3D         & HT    & 53.1 & 82.7  \\
	XDC~\cite{alwassel2019self}               & R(2+1)D-18  & IG65M & 56.0 & 85.3  \\
	MMV~\cite{alayrac2020selfsupervised}      & R(2+1)D-18  & AS    & 60.0 & 83.9  \\
	ELo~\cite{piergiovanni2020evolving}       & R(2+1)D-50  & Y8M   & 64.5 & --   \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-1em}
\caption{\textbf{Comparison to state-of-the-art.} Transfer learning results on UCF-101 and HMDB-51 when video backbone is frozen. \label{tab:sota_linear}}
\end{table}

==> STiCa (ICCV 2021)/tabs/sota_retrieval.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}
\centering
\footnotesize
  \begin{tabular}{lccc c  ccc}
  \toprule
       & \multicolumn{3}{c}{\textbf{UCF}} && \multicolumn{3}{c}{\textbf{HMDB}} \\
       \cmidrule{2-4} \cmidrule{6-8}
        \multicolumn{1}{r}{Recall @} & 1 & 5  & 20 && 1 & 5 & 20   \\
\midrule
    % SpeedNet~\cite{benaim2020speednet}       & 13.0 & 28.1 & 49.5  && --  & --   & --    \\
    % ST-Puzzle~\cite{kim2019self}             & 19.7 & 28.5 & 40.0  && --  & --   & --    \\
    % OPN~\cite{lee2017unsupervised}           & 19.9 & 28.7 & 40.6  && --  & --   & --    \\
    % ST Order ~\cite{buchler2018improving}    & 25.7 & 36.2 & 49.2  && --  & --   & --    \\
    %VCOP~\cite{clip_order}                   & 14.1 & 30.3 & 51.1  && 7.6 & 22.9 & 48.8  \\
    %VCP~\cite{luo2020video}                   & 18.6 & 33.6 & 53.5 && 7.6 & 24.4 & 53.6  \\
    MemDPC~\cite{Han2020MemoryaugmentedDP}   & 20.2 & 40.4 & 64.7  && 7.7 & 25.7 & 57.7  \\
    VSP~\cite{cho2020selfsupervised}         & 24.6 & 41.9 & 62.7  && 10.3& 26.6 & 76.8 \\
    SeLaVi~\cite{asano2020labelling}         & 52.0 & 68.6 & 84.5  && 24.8 & 47.6 &75.5 \\
    CoCLR~\cite{Han2020SelfsupervisedCF}     & 55.9 & 70.8 & 82.5  && 26.1 & 45.8  & 69.7  \\
    GDT~\cite{Patrick2020MultimodalSF}       & 57.4 & 73.4 & 88.1  && 25.4 & 51.4  & 75.0  \\
\midrule
    \textbf{Ours:  \methodname}                                      & $\bf{59.1}$ & $\bf{76.2}$ & $\bf{88.1}$  && $\bf{26.3}$ & $\bf{49.2}$  & $\bf{76.4}$  \\
\bottomrule
  \end{tabular}
%  \vspace{1em}
\vspace{-0.5em}
  \caption{\textbf{Comparison to SoTA for retrieval.} Nearest neighbor action retrieval performance @$k=\{1,5,20\}$.  \label{tab:ret}}
% \vspace{-1.5em}
\end{table}
 
 


==> STiCa (ICCV 2021)/tabs/supervised.tex <==
\begin{table}
\begin{center}

\begin{tabular}{cc}
\toprule
Fm-Crop & HMDB-51 Top-1 Acc. \\
\midrule
{\color{gray}\xmark} & 67.6 \\
\cmark               & 69.0 \\
\bottomrule
\end{tabular} 
\end{center} 
\vspace{0.5em}
\caption{\textbf{Supervised Training.} We train the R(2+1)D+Transformer architecture supervisedly on Kinetics-400 with and without feature crops enabled. \label{tab:ablation:supervised}}
\end{table}

==> STiCa (ICCV 2021)/vedaldi.tex <==
\newif\ifdark
\IfFileExists{/Users/vedaldi/.bash_profile}{
\immediate\write18{%
if defaults read -g AppleInterfaceStyle 2>/dev/null;
then echo \\darktrue > /tmp/displaymode.tex;
else echo \\darkfalse > /tmp/displaymode.tex; fi}
\input{/tmp/displaymode.tex}
\ifdark
\definecolor{pcolor}{HTML}{1E1E1E}
\definecolor{tcolor}{HTML}{C5C5C5}
\else
\definecolor{pcolor}{HTML}{FDF6E3}
\definecolor{tcolor}{HTML}{333333}
\fi
\pagecolor{pcolor}
\color{tcolor}
% Suppress hbadness warnings.
\hbadness=\maxdimen
\vbadness=\maxdimen
\vfuzz=30pt
\hfuzz=30pt
}{} 

==> tabs/abl_transformer_pos.tex <==
\begin{table}
\begin{center}

\begin{tabular}{cc}
\toprule
Pos Encoding.  & Acc. \\
\midrule
\xmark  & $62.7$ \\
\cmark  & $62.1$\\
\bottomrule
\end{tabular} 
\end{center} 
\caption{\textbf{Transformer Positional Encoding.} Positional encoding makes little difference in final performance. \label{tab:ablation:pos_encoding}}
\end{table}
